Empowering Dual-Level Graph Self-Supervised Pretraining with Motif Discovery

While self-supervised graph pretraining techniques have shown promising results in various domains, their application still experiences challenges of limited topology learning, human knowledge dependency, and incompetent multi-level interactions. To address these issues, we propose a novel solution, Dual-level Graph self-supervised Pretraining with Motif discovery (DGPM), which introduces a unique dual-level pretraining structure that orchestrates node-level and subgraph-level pretext tasks. Unlike prior approaches, DGPM autonomously uncovers significant graph motifs through an edge pooling module, aligning learned motif similarities with graph kernel-based similarities. A cross-matching task enables sophisticated node-motif interactions and novel representation learning. Extensive experiments on 15 datasets validate DGPM's effectiveness and generalizability, outperforming state-of-the-art methods in unsupervised representation learning and transfer learning settings. The autonomously discovered motifs demonstrate the potential of DGPM to enhance robustness and interpretability.

==> contents/8rebuttal.tex <==
\twocolumn
\noindent 
\textit{We appreciate all the reviewers for your thoughtful and helpful comments. Efforts will be made to enhance this work following your suggestions.
Here are responses and \textit{\textbf{R}} for \textbf{Reviewer}, \textit{\textbf{Q}} for \textbf{Question}, \textit{\textbf{W}} for \textbf{Weakness}.}

\textbf{To \textit{Q1} of \textit{R3} and \textit{Q1, Q2} of \textit{R5} about the model complexity:}
% R3Q1: 1. Could you elaborate on the computational complexity of the Motif Auto-Discovery process? How does it scale with the size and complexity of the graphs? [Model analysis-Complexity.]
% R5Q1: Complexity: The dual-level pretraining structure and motif discovery might increase the complexity of the model; the authors need to be specific on this. [Model analysis-Complexity.] 
% R5Q2: Generalization: Generalization: how does the approach generalize wrt the amount of data? [Model analysis-Complexity.] 
We provide a detailed analysis of the computational complexity of components in DGPM \textbf{in Appendix D}, including node feature reconstruction, motif auto-discovery, and node-motif cross-matching. The overall time complexity is $\mathcal{O}(|V|\log(|V|))$. Considering DGPM is a pretraining framework, we find this time complexity acceptable.
%We presented the computational complexity of DGPM \textbf{in Appendix D. }
% The time complexity of DGPM is analyzed by three components:
% 1. For \textbf{node feature reconstruction}, the time complexity is linear with the number of nodes $n$, that is $\mathcal{O}(|V|)$. 
% 2. For \textbf{motif auto-discovery}, the computational complexity depends on edge-pool process and graph similarity loss. 
% In edge-pooling process, the aggregation scores are computed and checked by edges, thus the computational complexity here is $\mathcal{O}(|E|)$. For graph similarity loss, as equation \(6\) in the Methodology part shows, the loss is measured by combination pairs of motifs, leading to a time complexity $\mathcal{O}(|\mathcal{M}|^2)$, $\mathcal{M}$ for the set of motifs. 
% 3. For \textbf{cross-matching part}, according to equation \(7\), the loss is computed on the permutation of nodes and motifs, thus having a time complexity $\mathcal{O}(|V||\mathcal{M}|)$.
% Given motifs are merged by nodes with an exponential rate, we have $\mathcal{|M|} \sim \log(|V|)$, \textbf{then the overall time complexity} of the DGPM framework is as $\mathcal{O}(|V|\log(|V|))$.
%In short, we analyzed the complexity of node feature reconstruction, motif auto-discovery, and node-motif cross-matching. The overall time complexity of DGPM framework is as $\mathcal{O}(|V|\log(|V|))$.

\textbf{To \textit{Q2} of \textit{R3} about dataset domains in Experiments:}
% R3Q2: 2. The paper mentions that DGPM is domain-agnostic. Have you tested its performance on graphs from significantly different domains, such as social networks and biological networks, to validate this claim?
We utilized 15 datasets from \textbf{four distinct domains} in our experiments, including social networks, citation networks, chemical compounds, and proteins. Details of these datasets are in \textbf{Appendix A} and will be highlighted in the revision.
%A detailed introduction of implemented datasets can be found in \textbf{Appendix A}. In short, datasets from \textbf{four domains} are included in the Experiments part, including \textbf{social networks, citation networks, chemical compounds, and proteins}.

\textbf{To \textit{Q3} of \textit{R3} and \textit{Q1, W1} of \textit{R4} about the details of node-motif matching task and feature-fusion method:}
% R3Q3: 3. The Cross-Matching Learning Module is a key component of DGPM. Could you provide more details on how the feature fusion is achieved and why this particular method was chosen?[Model technique details.]
% R4Q1: 1. How is the node-motif matching task implemented? [model technique details.]
% R4W1: 1. The section of the proposed method lacks details, resulting in an unclear explanation of certain methodological aspects.
% Based on dual-level pretraining, we obtained representations for nodes and subgraphs in each graph. 
In the \textit{node-motif matching task}, the inherent affiliation relationship between nodes and motifs is the learning objective. Specifically, we concatenate the normalized representations of nodes and motifs, and use that as a feature to predict the existence of the affiliations relationship. By performing this operation for each node, we achieved the learning of node-motif matching. Prior work (Wu et al. TKDE2021) has already demonstrated the direct and effective utility of employing affiliation relationships in cross-level pretraining tasks. The design of \textit{feature fusion approach} aims to align the pretraining with downstream tasks. The framework encodes nodes and motifs, combining them into a unified feature for downstream tasks. Specifically, we concatenate representations from different levels for classification. Prior studies, such as prompt learning (Liu et al. 2023), have demonstrated that incorporating tasks similar to the downstream tasks during the pretraining phase enhances adaptability. We will incorporate more details into our method. 

%\textbf{As illustrated in the top-left corner of Figure ~\ref{fig:model_framework}, node 1 belongs to motif A, not B. For node 1, two features are generated by concatenating representations of node 1 with the representations of motifs A and B, and the corresponding ground truth labels (colored in green) are 1 and 0 respectively.} 

%The inherent affiliation relationship between nodes and motifs is the learning objective in the node-motif matching task. Specifically, we concatenate the normalized representations of nodes and motifs, and use that as a feature to predict the existence of the affiliations relationship. \textbf{As illustrated in the top-left corner of Figure ~\ref{fig:model_framework}, node 1 belongs to motif A, not B. For node 1, two features are generated by concatenating representations of node 1 with the representations of motifs A and B, and the corresponding ground truth labels (colored in green) are 1 and 0 respectively.} By performing this operation for each node, we achieved the learning of node-motif matching.

%The affiliation relationship has been employed in cross-scale graph self-supervised learning to construct pretraining tasks~\cite{jiao2020sub,zhang2020motif,wu2021self}, as being simple, direct, and effective. \textbf{Besides, the design of taking concatenation as a feature fusion approach aims to align the pretraining with downstream tasks.} The learning strategy of this framework is to encode nodes and motifs and then combine them into one feature for downstream tasks. Therefore, we design to concatenate the representations of different scales and perform a classification task. Previous studies on pretrained models like prompt learning~\cite{liu2023pre} have shown that using similar or related tasks to the downstream tasks in the pretraining phase helps \textbf{improve the pretraining's adaptability.}

\textbf{To \textit{W1} of \textit{R3}:}
% R3W1: While the motif discovery is novel, the concept of self-supervised learning on graphs is not new. The paper could benefit from a more thorough discussion comparing it with existing methods in this area. [Literature Review]
We will include more related studies to facilitate a more comprehensive discussion.
%Depending on pretext task design, we discussed current self-supervised pretraining methods on graphs from contrastive learning and predictive learning\cite{hao2019visualizing,zoph2020rethinking} in Related Works on page 7. We will include more timely related works in the next version.

\textbf{To \textit{Q2} of \textit{R4} about the optimal number of EdgePool layers:}
% R4Q2: How do we determine the optimal number of layers to stack on EdgePool? As shown in Fig3, layers 2 and 3 demonstrate exceptional performance. [Model Analysis-Hyperparameter.] 
In \textbf{Sensitive Analysis} of \textbf{Experiments} section, we conducted a detailed analysis of the optimal number of EdgePool layers. We found the optimal number of EdgePool layers is contingent on the complexity of the graphs. Typically, 2-3 layers, capturing motifs with maximum sizes of 4-8, are good defaults for small graphs. We'll suggest the appropriate layer numbers based on our analysis. 
%A detailed analysis of the optimal number of EdgePool layers is presented in \textbf{Sensitive Analysis} of \textbf{Experiments} part. In short, the optimal number of EdgePool layers is related to the complexity of the motifs in graphs.

\textbf{To \textit{W2} of \textit{R4} about `node labels':}
% R4W2: Pretraining with Motif Discovery.' However, on page 4, it states that 'node labels serve as input features for MUTAG, PROTEINS, and NCI1 datasets.' This raises questions regarding the consistency and appropriateness of the title.
The term 'node labels' refers to node features, rather than the target label for pretraining i.e. affiliation of motifs.
% Sorry for the misunderstanding, we will employ more precise wording to address this distinction.
We will employ more precise wording to address this distinction.
%We are sorry for this ambiguous description. However, it should be clarified that the task is a graph-level classification task, and the "node labels" mentioned are features of nodes and have no direct relation to the targeted graph-level label.

\textbf{To \textit{W3} of \textit{R4}:}
% R4W3: 3. There are some typographical errors, notably, the incorrect marking of the optimal value for the MUTAG dataset in Table 1.
In Table 1, for the MUTAG, both InfoGCL and DGPM exhibit the same average accuracy. DGPM demonstrates a smaller standard deviation, indicating better stability. We will provide further clarification on this matter.
%We are sorry for the lack of explanation here. Here is not a typo because for models that have the same accuracy, the one that has a smaller standard deviation is better for a more stable performance. This is why we marked DGPM as the best on dataset MUTAG in Table 1.

\textbf{To \textit{Q3} of \textit{R5} about the model interpretability:}
% R5Q3: Interpretability: how can the motif be interpreted (e.g., visually) when their complexity increases? (I realize the edge pooling module is meant to limit the involvement of humans; still, humans need to interpret the results) [Model analysis-Interpretability]
% ~\cite{adler2022emergence}
Complex motifs can be viewed as combinations of simple motifs (Adler et.al PNAS2022). For DGPM, the motif discovery part stores the source nodes (subgraph) and the resulting subgraph for each merge, which can be visualized as an evolution process for each motif. We think this could help to explain where the complex motif from and possible properties based on the components included. 

\textbf{To \textit{W1} of \textit{R6} about the performance improvement:}
% R6W1: 1) It is proved that DGPM outperforms existing techniques for most cases. However, the improvement is small
% 拆开； 补一句，其他模型(具体哪几个文章（AAAI），在几个数据集上的提升在多少；)的提升；如果提升少，看某个数据集本身已有的表现；performance 放前面；
% For \textit{unsupervised representation learning}, Table 1 shows DGPM outperforms all unsupervised baselines across all datasets.
% For \textit{transfer learning}, Table~\ref{tab:table2} shows DGPM outperforms SOTA methods on 6 out of 8 datasets and achieves the best average performance.  
To validate the improvement of our model, apart from the performance reported in Table 1 and 2, we implemented two groups of \textbf{T-test} for two experimental settings. The tests show that both the performances of DGPM in these two settings are \textbf{significantly} (p\textless0.05) higher than that of other models.
Furthermore, we compared the \textbf{performance improvements} with other representative methods. Specifically, under the same task settings, we calculate the percentage of improvement between each target method and the baseline methods (in its original published paper): $\text{Improvement} = \left( \left( Acc_{\text{Target}}-Acc_{\text{Baseline}} \right )/ Acc_{\text{Baseline}} \right ) \cdot 100\%$. 
For the unsupervised learning graph classification setting, GraphMAE(KDD2022) shows an average improvement of 5.21±5.99\% (max: 27.88\%) on all baselines and datasets, whereas our method achieves an average improvement of \textbf{5.55±5.73\% (max: 28.12\%).}
For the transfer learning setting, D-SLA(NIPS2022) shows an average improvement of 4.44±5.72\% (max: 25.07\%), MOTIF(AAAI2021) achieves an average improvement of 2.19±1.79\% (max: 5.78\%) on all baselines and datasets, and our method achieves an average improvement of \textbf{4.30±4.85\% (max: 25.04\%).}
Note that most of the baselines for these compared models are the same as ours and we included newly published, stronger baselines in our paper.
Compared to prior published works, our method shows \textbf{similar or enhanced improvement} and \textbf{better model stability}. Given the enhancement over even more superior baselines, we find our model's performance improvement substantial.
% Furthermore, we compared the performance improvements with other representative methods. Specifically, under the same task settings, we calculate the percentage of improvement between each target method and the best-performing baseline method (in its original published paper) for each dataset: $\text{Improvement} = \left( \left( Acc_{\text{Target}}-Acc_{\text{BestBaseline}} \right )/ Acc_{\text{BestBaseline}} \right ) \cdot 100\%$. Note that the improvement could be negative as the target model may not outperform all baselines. For the transfer learning setting, \mark{D-SLA(NIPS2022) shows an average improvement of -0.16\% (max: 0.84\%, min: -1.60\%), MOTIF(AAAI2021) achieves an average improvement of 0.37\% (max: 1.01\%, min: -3.30\%) on all datasets,} and our method achieves an average improvement of 0.40\% (max: 1.34\%, min: -0.01\%). 
% For the unsupervised learning graph classification setting, GraphMAE(KDD2022) shows an average improvement of -0.37\% (max: 1.01\%, min:  -3.30\%) on all datasets, whereas our method achieves an average improvement of 0.39\% (max: 0.95\%, min: 0.00\%). Compared to prior published works, our method shows \textbf{similar or enhanced average improvement} and \textbf{better model stability}. Given the enhancement over even more superior baselines, we find our model's performance improvement substantial.
%This shows our method demonstrates comparable or even more significant performance improvement compared to published works.
%Considering that our method demonstrates enhancement in comparison to the already superior baseline models, we believe the performance improvement of our model is substantial.
%Furthermore, we compared the performance improvements with other representative methods. Specifically, under the same task settings, we calculate the percentage of improvement between each target method and the best-performing baseline method (in its original published paper) for each dataset, and then compute the average improvement for that method across all datasets:
% $$
% \text{Improvement} = \frac{1}{N}\sum_{i=1}^{N}\frac{Acc_{\text{prop}}-Acc_{\text{best w/o prop}}}{Acc_{\text{best w/o prop}} }\cdot 100\%
% $$
%(Note this index could be negative when the proposed model does not outperform across all datasets.)
% ~\cite{Subramonian_2021} ~\cite{NEURIPS2022_5b175f9e} \cite{hou2022graphmae}
% For the transfer learning setting with the same datasets as ours, the method proposed in (Subramonian AAAI2021) achieves an Improvement of 0.3714\%, and (Kim, Baek, and Hwang NIPS2022) shows an Improvement of -0.1631\%. In comparison, our method achieves an Improvement of 0.3985\%. 
% For the unsupervised learning graph classification setting with the same datasets as ours, (Hou et al. KDD2022) shows an Improvement of -0.3759\%, whereas our method achieves an Improvement of 0.3934\%.
% This shows our method demonstrates comparable or even more significant performance improvement compared to published works.

\textbf{To \textit{W2} of \textit{R6} about the model novelty:}
% R6W2: 2) The Design of DGPM is pretty simple and built on the top of existing technique. It is hard to see the novelty. My major concern is about the rough design of DGPM.
% contribution to the community, open source codes, interpretability.（potential）
%Firstly, we \textbf{innovatively propose a novel dual-level pretraining architecture} that enables the learning of both node and structural information by adapting to diverse network structures. Additionally, we \textbf{introduce the cross-matching-based affiliation prediction as a pretraining task}. This task facilitates the interplay between feature learning at different levels, providing mutual guidance while aligning with downstream tasks. Besides, the motif auto-discovery we proposed \textbf{improves the interpretability by visualizing motifs} in the pretraining process. To help other scholars reproduce the experiment and follow this work, we will \textbf{release the dataset and code.} We hope the AAAI audience will benefit from this work if this paper can be accepted.
This study addresses a series of critical challenges in graph pretraining: limited topology learning, human knowledge dependency, and incompetent multi-level interactions. To the best of our knowledge, this study is the \textbf{first} graph pretraining framework that utilizes a motif auto-discovery mechanism to leverage subgraph structure information in self-supervised learning. Meanwhile, we introduced the cross matching-based affiliation prediction as a \textbf{new pretraining task} to comprehensively learn the vital graph structures. Furthermore, our proposed method for automatic motif discovery has the potential to enhance the interpretability of the model, \textbf{offering fresh insights} into the capabilities of pretraining graph models in research. We will highlight these novelties and contributions in the revision.

\textbf{To comments of \textit{R5} on Significance and Quality:} WWL is employed to measure motif similarity as ground truth, guiding EdgePool layer training. A detailed introduction can be found in \textbf{Graph Similarity Loss} part of \textbf{Methodology} section. For the technical contribution, please refer to the response to \textit{W2} of \textit{R6}. Regarding the impact of DGPM, it is the first graph pretraining framework that utilizes a motif auto-discovery mechanism. We hope DGPM can not only enhance the performance of graph pretraining models but also assist in identifying crucial structural information in various domains. To facilitate reproducibility, we will make the dataset and code available to other researchers.
% Quality: The paper appers to be sound. Nevertheless, the connection with WWL needs to be made clearer. Moreover, the technical contribution per se is limited. The authors rearrange existing techniques. Even the edge pooling component has been already described in Oliver et al. 2022
% Significance: the technique appears interesting although the authors fail to provide further developments or hints about the broad impact of DGPM
% \textbf{R5W2: Further developments or hints about the broad impact of DGPM.}
 % WWL is employed to measure motif similarity as ground truth, guiding EdgePool layer training. A detailed introduction can be found in\textbf{ Graph Similarity Loss} part of \textbf{Methodology}.










